Decentralized Implicit Differentiation

The ability to differentiate through optimization problems has unlocked numerous applications, from optimization-based layers in machine learning models to complex design problems formulated as bilevel programs. It has been shown that exploiting problem structure can yield significant computation gains for optimization and, in some cases, enable distributed computation. One should expect that this structure can be similarly exploited for gradient computation. In this work, we discuss a decentralized framework for computing gradients of constraint-coupled optimization problems. First, we show that this framework results in significant computational gains, especially for large systems, and provide sufficient conditions for its validity. Second, we leverage exponential decay of sensitivities in graph-structured problems towards building a fully distributed algorithm with convergence guarantees. Finally, we use the methodology to rigorously estimate marginal emissions rates in power systems models. Specifically, we demonstrate how the distributed scheme allows for accurate and efficient estimation of these important emissions metrics on large dynamic power system models.

==> Appendices/NonSeparableConstraints.tex <==
\section{Non Separable Constraints}\label{appendix:non-separable}

==> Appendices/QP.tex <==
\section{Derivation for QPs}\label{appendix:QP}

In this section, as an exercise, we derive all relevant relationships in the general case of subproblems defined by QPs with linear constraints, and linear coupling constraints. That is, the general problem writes
\begin{align*}
    \min_{x_i} & \sum_i^N x_i^TP_ix_i + c_i^Tx_i\\
    \text{s.t. }& A_ix_i-b_i \preccurlyeq 0, \ i = 1, ...,\ N \\ 
   &  M\mathbf{x}-d = 0
\end{align*}
where the matrices $P_i$ are PSD, and the global coupling matrix $M = [m_1, m_2, ..., m_N]$. 

\paragraph{Local Jacobians} Let us take $\theta_i = (c_i, b_i)$ as the parameters we are interested in evaluating the sensitivity towards.
The local problems after writing the partial Lagrangian are $(i=1...N):$
\begin{align*}
    \min_{x_i} &\ x_i^TP_ix_i + c_i^Tx_i + \nu^Tm_ix_i\\
    \text{s.t. }& A_ix_i-b_i \preccurlyeq 0
\end{align*}
Writing $z_i = (x_i, \lambda_i)$ where $\lambda_i$ is the \textit{local} dual variable, and $\bar{\theta}_i = [\theta_i, \nu]$, the KKT matrix $g_i$ writes
$$
g_i = 
\begin{bmatrix}
c_i + m_i^T\nu + A_i^T\lambda_i + P_ix_i\\
diag(\lambda_i)(A_ix_i-b_i)
\end{bmatrix}, 
$$
and we have
$$
\partial_{z_i}g_i(z_i, \bar{\theta}_i) =
\begin{bmatrix}
    P_i & A_i^T\\
    diag(\lambda_i)A_i & diag(A_ix_i-b_i)
\end{bmatrix} \in \mathbbm{R}^{(n+l) \times (n+l)}.
$$
Given the chosen parameters, we have
$$
\partial_{\bar{\theta}_i}g_i = 
\begin{bmatrix}
    I & 0 & m_i^T \\
    0 & -diag(\lambda_i) & 0
\end{bmatrix} \in \mathbbm{R}^{(n+l) \times (n+l+\Lambda)}.
$$
Once we have computed these quantities, we  can solve
\begin{align}
    \partial_{\bar{\theta}_i}x_i &= - (\partial_{z_i}g_i(z_i, \bar{\theta}_i))^{-1}\partial_{\bar{\theta}_i}g_i \\
    & = [\partial_{\theta_i}x_i, \partial_{\nu}x_i]
\end{align}

\paragraph{Consensus} We are now in position to compute $\partial_{\pmb{\theta}}\nu$ given Eq.~\eqref{eq:consensus}. We can gather all local jacobians computed above and,
rewriting this equation with the appropriate variables, 
\begin{equation}
    \partial_{\pmb{\theta}}\nu = -(M\partial_\nu \mathbf{x})^{-1}M\partial_{\pmb{\theta}}\mathbf{x}
\end{equation}
Under the current assumptions of independence of parameters and local primal variables, we note that $\partial_{\theta_j}x_i = 0$ for $ i \neq j$. Note that the matrix $M\partial_\nu \mathbf{x} \in \mathbbm{R}^{\Lambda \times \Lambda}$.

\paragraph{Updating local Jacobians}
The final step is to compute the total derivative of the local variables wrt local parameters according to Eq.~\eqref{eq:update_local}:

\begin{align}
   D_{\theta_i}x_i^\star(\theta_i, \nu) = \partial_{\theta_i} x_i^\star + \partial_{\nu}x_i^\star \partial_{\theta_i}\nu 
\end{align}

==> Appendices/Self-dual.tex <==
\section{Derivation via self-dual embeddings}\label{appendix:self-dual}

\subsection{Cone constraints}
General cone constraints present a different challenge. Indeed, according to Amos, we cannot easily differentiate through the KKT because of the cone constraints. \textbf{I DON'T UNDERSTAND WHY THAT IS THE CASE YET, BUT LET'S WALK WITH THIS ASSUMPTION FOR NOW}

If this is true, we need a generalization of the KKT condition to differentiate through so that the framework is applicable to also SOCP, SDP, etc. To enable this, we borrow from Ye, Besutti, O'Donohue, Agrawal and Amos (5 different papers). These papers rely on an embedding proposed by Ye to implicitly define the solution. Basically, it is another set of conditions that the solution needs to satisfy, and relies on a few properties.

I will illustrate my thinking roughly here, and polish the text later.

First of all, the above logic still applies. Namely, we can write the Lagrangian containing the objective function and the coupling constraint. At optimality, every local problem solves the local objective + part of the term that involves the coupling constraint, s.t. local constraints. So, basically, the proposed logic still applies. 

Second, we differentiate locally, also as exposed. \textbf{Note: If the local problem is a cone program, we can differentiate through it given methods exposed in mentioned papers (Amos, Agrawal). It is important to state that the only thing we do, locally, is differentiate as is already known in the literature - but we differentiate with the objective being the augmented Lagrangian, and wrt extended parameters}. 

We have so far expressed how to compute the coupling jacobian in the case of equality or inequality constraints. This logic simply relied on differentiating through the KKT conditions. However, it is not as easy to do if the coupling constraint is of the form
\begin{align*}
h_i(x) \preccurlyeq_{\mathcal{K_i}} 0, \ i =1, ... \Lambda
\end{align*}
with $\mathcal{K}$ being a second-order cone, a semi definite cone, exponential cone, etc. This said, we should intuitively still be able to perform a similar operation, that is, express the gradient of the dual coupling variable as a function of individual gradients, and correct the local gradients on this basis.

\subsubsection{Homogeneous self-dual embedding}

Similarly to the above mentioned papers, we propose to build an embedding of the coupling constraint and coupling dual variable: 
\begin{align*}
Q = \begin{bmatrix} 
0 & H(x) \\
- H(x)^T & 0
\end{bmatrix}
\end{align*},
where $H(x)^T = [h_1(x), ... h_\Lambda(x)]$. \textbf{If we have a solution} (here the goal is not to find a solution, we assume we have an appropriate solution to the problem), then we construct two vector $u, v$ such that $u = (\lambda, 1), v = (s, 0)$, where $\lambda = [\lambda_1, ... \lambda_\Lambda]$ is the vector of dual variables associated with the coupling constraints and $s = [s_1, ... s_\Lambda]$ is the primmal slack variable associated to those cone constraints. This implies
\begin{itemize}
    \item $Qu = v$ (i.e. the coupling constraint is satisfied as well as the associated complementary slackness condition)
    \item $ u \in \bar{\mathcal{K}}, \bar{\mathcal{K}} = \mathcal{K}^\star \times \mathbb{R}_+$; $v \in \bar{\mathcal{K}}^\star, \in \bar{\mathcal{K}}^\star = \mathcal{K} \times \mathbb{R}_+$. Therefore, both $u, v$ belong to cones that are mutually dual! Indeed, the nonnegative orthant is self dual \textbf{I think?}. 
    \item $u^Tv = 0$, i.e. $u, v$ belong to complementary vector spaces in $\mathbb{R}^\Lambda$
\end{itemize}

Given those properties, we can use the theorem of Moreau that enables decomposition of an element of a hilbert space over the conic complementary set. Namely, we have that
\begin{align*}
    z = u - v\\
    u = \Pi_{\bar{\mathcal{K}}} z, v = - \Pi_{\bar{\mathcal{K}}^\star} z\\ 
    \Rightarrow \Pi_{\bar{\mathcal{K}}} = I - \Pi_{\bar{\mathcal{K}}^\star}
\end{align*}

For simplicity, we will denote $\Pi_{\bar{\mathcal{K}}}$ simply by $\Pi$ in the remainder of the document. 

Therefore, we can rewrite the condition that $u, v$ satisfy as
\begin{align*}
    Q\Pi z + (I - \Pi)z = 0 \\ 
    ((Q - I)\Pi + I) z = 0 = \mathcal{R}(z)
\end{align*}
$\mathcal{R}(z)$ denotes the residual map. It is supposed to be $0$ for any solution embedded in the above way.

\subsubsection{Derivation through the embedding}
The above embedding provides a map $\mathcal{R}(z)$ that is different from the KKT conditions but is differentiable. Once it is constructed, the only thing we need is to do is apply the same mechnanics as before. 

The only thing we want to recover is the Jacobian $D_\theta \lambda =[I, 0] D\Pi (z) D_\theta z = [\Pi_{\mathcal{K}^\star},\ 0]D_\theta z$ (\textbf{note} that we are projecting on the dual cone, because we want to recover the dual variables).  Therefore, we can recover the gradient of the dual variable by projecting the gradient of $z$. 

We apply the implicit differentiation theorem, again. 

\begin{align*}
    \partial_\theta z = - (\partial_z \mathcal{R}(z))^{-1} \partial_\theta \mathcal{R}(z)
\end{align*}

We can analyze both terms in this equation:
\begin{itemize}
    \item $\partial_z \mathcal{R}(z) = \partial_z Q \Pi z + (Q- I) \partial_z (\Pi z) + I$\\
    \item $\partial_\theta \mathcal{R}(z) = \partial_\theta Q \Pi z$
\end{itemize}

Computing $\partial_z Q$ is the new part here. Let's note that $\partial_z x_i(\theta, \lambda(\theta)) = \partial_\lambda x_i \partial_z \lambda = \partial_\lambda x_i [I, 0] D\Pi$, as $\lambda = [I, 0] \Pi z$. This allows the derivation of the matrix $Q$ wrt $z$. The rest should not be an issue. Similarly, we can compute $\partial_\theta Q$ by taking the derivatives directly for each component of the matrix.

\subsubsection{Ensuring invertibility}

As we have seen, we need the last component of $z$ to ensure complementary slackness but we never recover the information at that level. Indeed, $\lambda = [I, 0] \Pi z$. Therefore, we only need ``all the rows but the last one'' of the inverse of the residual map. I have some hints indeed that it might now always be differentiable \textbf{why?}. Therefore, we can construct only the first row of the inverse of the matrix (by block decomposition), multiply it by the RHS, and then project on the dual cone without ever thinking about the last component of $z$. 



==> Appendices/SuppFigs.tex <==
\section{Supplementary Figures}\label{appendix:supp_figs}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.5\textwidth]{Figures/Scaling/ρ_fixed_th0.8_speedup.pdf}
    \caption{Scaling of the computational gain for a fixed number of coupling constraints $\Lambda=2$, and for different sizes of subproblems, with the central problem represented as a sparse matrix.}
    \label{supp_fig:scaling_sparse}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=.4\textwidth]{Figures/BatteryModel/cost.pdf}
    \caption{Caption}
    \label{supp_fig:cost}
\end{figure}

==> body/3.Distributed.tex <==
\section{Distributed Implicit Differentiation in Graph-Structured Problems}\label{sec:distributed}

In this Section, we adapt these schemes to enable a fully distributed solution of the coupling Jacobian in~\eqref{eq:coupling_gradients}. In Section~\ref{sec:graph_properties} we review relevant results from~\cite{Shin2020-jc, Shin2022-jo}. Then, in Section~\ref{sec:fully_dist_gradient} we describe the application of the distributed scheme in~\cite{Shin2020-jc} to our problem. We prove that they apply directly to the system in~\eqref{eq:coupling_gradients} under the conditions of Theorem~\ref{th:DID}.

\subsection{Graph-induced matrix properties}\label{sec:graph_properties}

A \textit{graph-structured matrix} is a matrix whose structure derives from an associated graph. The connectivity of the graph will result in a generalization of the notion of \textit{bandwidth} on this matrix.

\begin{definition}[Graph-Induced Bandwidth] 
Consider a matrix $X \in \R^{m \times n}$, a graph $\G = (\V, \E)$, and index sets $\mathcal{I} = \{I_i \}_{i \in \V }$ and $\mathcal{J} = \{J_i \}_{i \in \V}$ that partition $\mathbb{I}_{[1, m]}$ and $\mathbb{I}_{[1, n]}$, respectively. 
Matrix $X$ is said to have bandwidth $B_X$ induced by $(\G, \mathcal{I}, \mathcal{J})$ if $B_X$ is the smallest nonnegative integer such that $X_{[i][j]} = 0$ for any $i, j \in \V$ with $d_{\G}(i,j) > B_X$, where $X_{[i][j]} = X_{\mathcal{I}_i, \mathcal{J}_j}$.
\end{definition}
In the above definition, the distance on the graph $d_{\mathcal{G}}(i, j)$ between two nodes $i, j$ is the number of edges on the shortest path connecting them in $\mathcal{G}$. If the bandwidth of a matrix is much smaller than the diameter of the associated graph (i.e. the maximum distance between two nodes on the graph), one talks about a \textit{graph-induced banded matrix.} We now recall the main result of~\cite{Shin2022-jo}.

% In the affine case, the coupling constraints in~\eqref{eq:coupling_constraints} are $H_i(x_i, \theta_c) = h_i(\theta_c) x_i$ and $F_i(x_i, \theta_x) = f_i(\theta_c) x_i$. 


% mention the interpretation of the bipartite graph, maybe draw it, and link it with the bandedness of the matrix. basically it is constraints sharing a similar node, this is why the bandwidth increases
% two ideas to put forward
% - here the system we are trying to solve is structured from a constraint-constraint graph
% - however, underlying that graph, there is a bipartite graph that links subproblems to constraints


% from now on, we will write the coupling equation as
% L D_\theta u = q

% first define the set of nodes and the distance \omega

% In our context, those graph-banded properties are important if the constraint matrices in Eq.~\eqref{eq:coupling_constraints} are structured. For instance, consider the case of dynamic optimization problems. The global problem represents a dynamical system made up of $T$ individual subproblems. In this context, the $T$ subproblems constitute a linear graph---i.e. a chain---and subproblem $t$ is involved in constraints with subproblems $t-1$ and $t+1$ only. Therefore, the sets of indices $\mathcal{I}, \mathcal{J}$ will represent ...


% \begin{lemma}\label{lemma:graph_rules}
% Consider $X\in\R^{m \times n}$ with bandwidth not greater than $B_X$ induced by $(\G, \I, \J)$; we have that (a) if $Y \in \R^{m \times n}$ has bandwidth not greater than $B_Y$ induce by $(\G, \I, \J)$, then $X+Y$ has bandwidth not greater than $\max(B_X, B_Y)$ induced by $(\G, \I, \J)$; (b) if $W \in \R^{n \times k}$ has bandwidth not greater than $B_W$ induced by $(\G, \J, \mathcal{K})$, then $XW$ has bandwidth not greater than $B_X + B_W$ induced by $(\G, \I, \mathcal{K})$. 
% \end{lemma}

\begin{theorem}[Theorem 3.6 in~\cite{Shin2022-jo}]
    \label{th:inverse_structure}
    Consider a nonsigular matrix $X \in \R^{n \times n}$ with bandwidth not greater than $B_X \geq 1$ induced by $(\G, \mathcal{I}, \mathcal{J})$. For constants $\bar{\sigma}_X \leq \bar{\sigma}(X)$ and $0 \leq \ubar{\sigma}_X \leq \ubar{\sigma}(X)$, the following holds
$$
\|X^{-1}_{[i][j]} \| \leq \frac{\bar{\sigma}_X}{\ubar{\sigma}^2_X}
\left(\frac{\bar{\sigma}_X^2 - \ubar{\sigma}^2_X}{\bar{\sigma}_X^2 + \ubar{\sigma}^2_X}\right)^{\left\lceil\frac{d_{\G}(i,j) - B_X}{2B_X}\right\rceil_+},
$$    
where $X^{-1}_{[i][j]} = X^{-1}_{\I_i, \J_j}$, $\bar{\sigma}(X), \ubar{\sigma}(X)$ denote the largest and smallest singular values of $X$, and $\left\lceil \cdot \right\rceil_+$ is the smallest non-negative integer that is greater than or equal to the argument.
\end{theorem}

% older version

% \begin{theorem}[Theorem 1 in~\cite{Shin2020-jc}]\label{th:inverse_structure}
%     Consider a PD matrix $H \in \mathbb{R}^{n\times n}$ and a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with $\{1, 2, \cdots, N \} \subseteq \mathcal{V}$. Suppose that any eigenvalue of $H$ satisfies $\lambda \in [\lambda_{\min}, \lambda_{\max}]$ for some $\lambda_{\min}, \lambda_{\max} \in \mathbb{R}_{0+}$. Then the following holds for any $i, j \in \{1, 2, \cdots, N \}$.
%     $$
%     \left|\left(H^{-1}\right)_{i,j} \right| \leq \frac{1}{\lambda_{\min}} 
%     \left(
%     \frac{\lambda_{\max} - \lambda_{\min}}{\lambda_{\max} + \lambda_{\min}}
%     \right)^{d_G(i, j)/\mathcal{B}_{\mathcal{G}}(H)}
%     $$
% \end{theorem}




% \begin{theorem}[Theorem 4 in~\cite{Shin2020-jc}]
% \label{thm:inverse_structure}
%     Consider a matrix $H\in \mathbb{R}^{n \times n}$ and a graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with $\{1, 2, \cdots, N \} \subseteq \mathcal{V}$. Suppose that the eigenvalues of $H$ are in $\{\lambda \in \mathbb{C} | |\lambda - z| \leq R\}$ for some radius $R \in \mathbb{R}_{0+}$ and $z \in \mathbb{C} \setminus \{ 0\}$ such that $R < |z|$. For any given $\varepsilon \in (0, 1-R/|z|)$, there exists $C = C(H, \varepsilon) \in \mathbb{R}_{0+}$ such that
%     \begin{align*}
%     \left|\left( 
%     \left(
%     I - \frac{1}{z}H
%     \right)^m
%     \right)_{i,j} \right| \leq C \left(\frac{R}{|z|} + \varepsilon \right)^m
%     \end{align*}
%     holds for any $i, j\in \{1, 2, ..., N\}$ and $m\in\mathbb{Z}$. Furthermore, for such $C$ and $\varepsilon$, the following holds for any $i,j\in\{1, 2, ..., N\}$:
%     \begin{align*}
%         | (H^{-1})_{i,j}| \leq \frac{C}{(1-\varepsilon)|z| - R} \left( \frac{R}{|z|} + \varepsilon \right)^{d_{G}(i,j)/B_H}.
%     \end{align*}
% \end{theorem}

This theorem states that the inverse of a graph-structured matrix has exponentially decaying components. The magnitude of the $i,j$-th component of its inverse decreases exponentially with respect to the distance of nodes $i,j$ in the graph $\mathcal{G}$. In addition, the rate of decrease depends on the conditioning of the matrix. 

% Those generic results rely on the condition that the matrix considered be PD, even though a similar result holds for any matrix with finite spectral radius (see Theorem 4 in~\cite{Shin2020-jc}). The following two results establish that the system in~\eqref{eq:coupling_gradients}, and therefore that the above theorem applies to our setting.


% This is false
% \begin{lemma}
%     \label{lemma:coupling_jacobian_PD}
%     If an optimization problem in the form of~\eqref{pbm:CCOP} satisfies Assumptions~\ref{A1},~\ref{A2},~\ref{A4} \&~\ref{A5} and if every subproblem is strictly convex, then the coupling Jacobian $\partial C$ in~\eqref{eq:coupling_gradients} is Positive Definite (PD).
% \end{lemma}
% The proof is provided in Appendix~\ref{proof:coupling_jacobian_PD}.


\subsection{Distributed Computation}\label{sec:fully_dist_gradient}

In this Section, we adapt the synchronous decentralized algorithm from~\cite{Shin2020-jc} to solve the coupling system in~\eqref{eq:coupling_gradients} in a fully distributed fashion. The method exposed in~\cite{Shin2020-jc} initially relies on the matrix to be inverted to be Positive Definite (PD). The coupling Jacobian of interest here is not necessarily PD because it is not symmetric if there are coupling inequality constraints. However, we show that the methodology readily applies to our system thanks to Theorem~\ref{th:inverse_structure} and the specific structure of the coupling Jacobian (see Lemmas~\ref{lemma:banded} \&~\ref{lemma:Lkw_invertible} below).

% The complication in DID is to compute the coupling jacobian. This requires solving the linear system in Eq.~\eqref{eq:coupling_gradients}. We will show that, for graph-structured coupling constraints, this coupling jacobian benefits from the above mentioned properties that can be used to design fully distributed algorithms. 


% The system in Eq.~\eqref{eq:coupling_gradients} is of dimension $\Lambda \times \Lambda$. 
% An element $(\partial G_c)_{i,j}$ is nonzero if constraints $i,j$ share a mutual connection, i.e. if there is at least one subproblem involved in both constraints. 

In our context, we are inherently dealing with a bipartite graph $\G_b$ inducing structure on the coupling system of Eq.~\eqref{eq:coupling_gradients}. The nodes of the graph can be separated in a set $\mathcal{V}_p$ of subproblems with $|\mathcal{V}_p| = N$ and $\mathcal{V}_c$ of constraints with $|\mathcal{V}_c| = \Lambda_H + \Lambda_F$. Each subproblem is linked to others indirectly via constraints. This graph directly induces structure on $\lhs$. Indeed, let us consider the matrix
$M_C = \begin{bmatrix}
    \partial_{\mathrm{x}} H^T & \partial_{\mathrm{x}} F^T
\end{bmatrix}^T.$ 
The structure of $M_C$ reflects the relationship between subproblems, and is linked to the structure of the coupling Jacobian as stated by the following Lemma.

\begin{lemma}\label{lemma:banded} 
Consider the graph $\G_b$ and define the index sets $\mathcal{I} = \{I_i\}_{i \in \V_c}$ and $\mathcal{J} = \{J_i\}_{i \in \V_p}$ that partition the set of constraints $\mathbb{I}_{[1, \Lambda]}$ and the set of subproblems $\mathbb{I}_{[1, N]}$, respectively.
If $B_{M_C}$ denotes the bandwidth of $M_C$ induced by $(\G_b, \I, \J)$ and $B_\lhs$ the bandwidth of $\lhs$ induced by $(\G_b, \I, \I)$, then $B_{\lhs} \leq 2 B_{M_C}$.
\end{lemma}
The proof is provided in Appendix~\ref{proof:banded}. The above result states that if the matrices encoding the coupling constraints in Eq.~\eqref{eq:coupling_constraints} are \textit{graph-induced banded} (i.e. have a small bandwidth compared to the overall size of the related graph $\G_b$), the LHS of Eq.~\eqref{eq:coupling_gradients} is itself banded with a bandwidth at most twice the bandwidth of the constraint matrices. Actually, $\lhs$ has the same structure as the Laplacian of the graph $\G_b$.


To each subproblem $k \in \mathcal{V}_p$, we now associate a restricted number of constraint nodes in the bipartite graph
$$
\mathcal{V}_k^\omega = \{c \in \mathcal{V}_c \ |\  d_{\G_b}(c, k) \leq 2\omega +1\}.
$$
The parameter $\omega \in \mathbb{Z}$ quantifies how far in the graph the constraints considered are from a given subproblem. For instance, $\mathcal{V}_k^0$ is the set of constraints that subproblem $k$ is directly involved in. 
If the coupling constraints in~\eqref{eq:coupling_constraints} are structured and sparse, each subproblem in $\V_p$ will be linked to only a few constraints. Therefore, the Jacobians $\partial_\nu x_i$ and $\partial_\mu x_i$ will also be sparse. Namely, they will be nonzero only at the columns corresponding to the constraints subproblem $i$ is directly involved in, i.e. $\V_k^0$. Subproblem $k$ thus only requires the coupling Jacobians $D_\theta \nu, D_\theta \lambda$ for the constraints in $\V_k^0$.

We define a set of projections for each subproblem $k$ and value of $\omega$ as follows:
(a) $T_k := \{e_i \}_{:, i\in \mathcal{V}_k^0 }$ is the projection on the set of constraints that subproblem $k$ is directly involved in; 
(b) $T_k^\omega := \{e_i \}_{:, i\in \mathcal{V}_k^\omega }$ is the projection on the set of constraints that subproblem $k$ is at distance $2\omega+1$ from; 
(c) $T_{-k}^\omega := \{e_i \}_{:, i\in \mathcal{V}_c\setminus \mathcal{V}_k^0 }$ is the projection on the set of constraints that subproblem $k$ is further than a distance $2\omega+1$ from. From there, we have
\begin{align}
\label{eq:projections}
\begin{array}{rl}
    \lhs^\omega_k &:= (T^\omega_k)^T \lhs T^\omega_k,\\ 
    \lhs^\omega_{-k} &:= (T^\omega_k)^T \lhs T^\omega_{-k},\\
    q^\omega_k &:= (T_k^\omega)^Tq.
\end{array}
\end{align}
The above matrices are the projections of the original system onto the set of constraints specified by $\mathcal{V}_k^\omega$. 
Constructing the local projections from~\eqref{eq:projections} does not require constructing the entire LHS matrix $\lhs$. Indeed, $\lhs$ is a sum of local components as shown in~\eqref{eq:coupling_gradients_sum}, and only a limited number of terms are required to construct this local projection. Denote by $\mathcal{P}_k^\omega = \{ i \in \mathcal{V}_p \ | \ d_\G(i, \mathcal{V}_k^\omega) \leq 1\}$ the set of subproblems that are directly involved in at least one of the constraints in $\mathcal{V}_k^\omega$. In other words, those are the subproblems at a distance less or equal to $2(\omega + 1)$ on the bipartite graph. As $T_k^\omega$ are nonzero only for the constraints in $\V_k^\omega$, the projections in~\eqref{eq:projections} can be limited to the local projections from $\mathcal{P}^\omega_k$, that is
\begin{align}
\label{eq:communication}
\begin{array}{rl}
\lhs^\omega_k &=  \sum_{i \in \mathcal{P}^\omega_k} (T^\omega_k)^T \lhs_i T^\omega_k,\\
\lhs^\omega_{-k} &=  \sum_{i \in \mathcal{P}^\omega_k} (T^\omega_k)^T \lhs_i T^\omega_{-k},\\
q_k^\omega &= \sum_{i \in \mathcal{P}^\omega_k} (T^\omega_k)^T q_i.
\end{array}
\end{align}
Constructing the projections thus only requires collecting data from a limited set of subproblems $\mathcal{P}_k^\omega$. In addition, if $\omega$ is small compared to the graph diameter, then the dimension of those matrices is small compared to the full coupling Jacobian. Subproblems must exchange matrices of sizes $|\V_k^\omega| \times |\V_k^\omega|$ instead of $\Lambda \times \Lambda$. Based on these projections, and assuming we have an estimate $y^{(t)}$ of the coupling Jacobian at iteration $t$, the next iteration of the decentralized scheme can be written as
\begin{align}
\label{eq:iteration}
    y_k^{(t+1)} = S_k^\omega y^{(t)} + U_k^\omega q,
\end{align}
where $y_k=\{y_j\}_{j \in \mathcal{V}_k^0}$  are the components of the coupling Jacobian corresponding to the constraints subproblem $k$ is directly involved in, and where
\begin{align}
    S_k^\omega &:= - (T_k)^T T_k^\omega (\lhs_k^\omega)^{-1} \lhs_{-k}^\omega (T_{-k}^\omega)^T, \\
    U_k^\omega & := (T_k)^TT_k^\omega(\lhs_k^\omega)^{-1}(T_k^\omega)^T.
\end{align}

This scheme can be interpreted as a \textit{block-Jacobi} method. In the iteration in Eq.~\eqref{eq:iteration}, subproblem $k$ updates the value of the coupling Jacobian associated to the constraint set $\mathcal{V}_k^\omega$ and keeps only the values associated to the constraints it is directly involved in. For this iteration to be well-defined, the local projections $\lhs_k^\omega$ need to be invertible.

\begin{lemma}
    \label{lemma:Lkw_invertible}
    Consider a constraint-coupled problem in the form of Problem~\ref{pbm:CCOP} an associated optimal solution $z^\star = (x^\star, \lambda^\star, \nu^\star)$. If the problem is strictly convex and satisfies Assumptions~\ref{A1},~\ref{A2},~\ref{A4} \&~\ref{A5}, then the projections $\partial C_k^\omega$ are invertible.
\end{lemma}
The proof is given in Appendix~\ref{proof:Lkw_invertible}. This result justifies the application of~\eqref{eq:iteration} to our problem. However, the algorithm detailed in~\cite{Shin2020-jc} assumes that the sets $\V_k^0$ are disjoint. In our case, they are inherently overlapping as, by definition, any coupling constraint links at least two subproblems together. The results of iteration~\eqref{eq:iteration} thus need to be aggregated for every constraint across each subproblem. We define an aggregation matrix $\Gamma \in \R^{\Lambda \times \sum_k |\V_k^\omega|}$ that simply averages the results across all nodes involved in each constraint such that $\Gamma_{i,j} = \frac{1}{\delta_i}$, with $\delta_i$ the degree of the constraint node $i$, if $j$ corresponds to a constraint that shares a subproblem with $i$.
% $\Gamma_{i,\J_k(j)} = \frac{1}{\delta_i} \mathbbm{1}\{k \in \mathcal{N}(i)\}$, ...
The resulting decentralized scheme is
\begin{align}\label{eq:sync_coord}
    y^{(t+1)} = \Gamma(S^\omega y^{(t)} + U^\omega q),
\end{align}
where
\begin{align*}
    S^\omega =
    \begin{bmatrix}
        (S^\omega_1)^T, ..., (S^\omega_N)^T
    \end{bmatrix}^T,\\
    U^\omega = \begin{bmatrix}
        (U^\omega_1)^T, ..., (U^\omega_N)^T
    \end{bmatrix}^T.
\end{align*}

For convergence, we need $\rho(\Gamma S^\omega) < 1$. As the spectral radius $\rho(\cdot)$ satisfies $\rho(\cdot) \leq \|\cdot \|_\infty$ ~\cite{Horn1990-ea} and the $\|\cdot\|_\infty$ is a matrix norm, it is submultiplicative and
$\rho(\Gamma S^\omega) \leq \| \Gamma S^\omega \|_\infty \leq \| \Gamma \|_{\infty} \|S^\omega\|_\infty \leq \| S \|_{\infty}$ as $\| \Gamma \|_{\infty} = 1$. The criteria derived in~\cite{Shin2020-jc} for convergence can therefore be readily applied to our setting.

\begin{theorem}[Adapted from Theorem 2 in~\cite{Shin2020-jc}]\label{th:convergence_rate}
Consider~\eqref{eq:coupling_gradients} and the decentralized scheme in~\eqref{eq:sync_coord} for a given set of node-associated constraint sets $\{\V_k^\omega\}_{k\in \V_p}$ and $\omega \geq 0$. Assume that the conditions of Lemma~\ref{lemma:Lkw_invertible} are verified. Then the sequence generated by~\eqref{eq:coupling_gradients} satisfies
\begin{align}
    \|y^{(t)} - y^\star \|_{\infty} \leq \alpha^t \|y^{(0)} - y^\star \|_\infty,
\end{align}
where the convergence rate $\alpha$ is defined by
\begin{align}
    \label{eq:alpha}
   \alpha := \max_{k \in \V_p} \frac{R_k \bar{\sigma}_k}{\ubar{\sigma}^2_k}  
   \left(
   \frac{\bar{\sigma}^2_k - \ubar{\sigma}^2_k}{\bar{\sigma}_k^2 + \ubar{\sigma}_k^2}
   \right)^{\left\lceil(\omega)/2B_{\lhs_k^\omega} - 1\right\rceil_+},
\end{align}
with $\bar{\sigma}^2_k$ and $\ubar{\sigma}^2_k$ the largest and smallest singular values of $\lhs_k^\omega$, respectively, and 
$R_k := \sum_{i \in \V_k^\omega, j \in \V \setminus \V_k^\omega} |(\lhs^\omega_{-k})_{i,j}|$.
\end{theorem}

The above result is a restatement of Theorem 2 in~\cite{Shin2020-jc}, without the assumption that the matrix be PD. As most steps in the proof remain unchanged, we do not rewrite it here entirely. We discuss the main differences in Appendix~\ref{proof:convergence_rate}.

The sequence~\eqref{eq:sync_coord} defines a scheme with linear convergence to solve~\eqref{eq:coupling_gradients}. The convergence rate $\alpha$ decreases exponentially with $\omega$. We note that for a given value of $\omega$, the conditioning as well as the graph-induced structure of the system will also impact $\alpha$. However, larger values of $\omega$ will come at a cost of more expensive communication, as more data needs to be exchanged both for constructing the projection matrices $\lhs_k^\omega, \lhs_{-k}^\omega, q_k^\omega$ and for the exchange of information at every iteration. In addition, the computational cost of one iteration of~\eqref{eq:sync_coord} increases with $\omega$. However, as $S_k^\omega$ remains unchanged with iterations, the factorization of $\lhs_k^\omega$ can be stored and does not need to be recomputed every time. 



==> body/3c.Distributedv3.tex <==
% version of the distributed section that is a trimmed down version of the original one.

% I keep it here to get some ideas for structuring it all

\subsection{Graph-induced matrix properties}\label{sec:graph_properties}

A \textit{graph-structured matrix} is a matrix whose structure derives from an associated graph. The connectivity of the graph will result in a generalization of the notion of \textit{bandwidth} on this matrix.

\begin{definition}[Graph-Induced Bandwidth] 
Consider a matrix $X \in \R^{m \times n}$, a graph $\G = (\V, \E)$, and index sets $\mathcal{I} = \{I_i \}_{i \in \V }$ and $\mathcal{J} = \{J_i \}_{i \in \V}$ that partition $\mathbb{I}_{[1, m]}$ and $\mathbb{I}_{[1, n]}$, respectively. 
Matrix $X$ is said to have bandwidth $B_X$ induced by $(\G, \mathcal{I}, \mathcal{J})$ if $B_X$ is the smallest nonnegative integer such that $X_{[i][j]} = 0$ for any $i, j \in \V$ with $d_{\G}(i,j) > B_X$, where $X_{[i][j]} = X_{\mathcal{I}_i, \mathcal{J}_j}$.
\end{definition}
In the above definition, the distance on the graph $d_{\mathcal{G}}(i, j)$ between two nodes $i, j$ is the number of edges on the shortest path connecting them in $\mathcal{G}$. If the bandwidth of a matrix is much smaller than the diameter of the associated graph (i.e. the maximum distance between two nodes on the graph), one talks about a \textit{graph-induced banded matrix.} We now recall the main result of~\cite{Shin2022-jo}.

\begin{theorem}[Theorem 3.6 in~\cite{Shin2022-jo}]
    \label{th:inverse_structure}
    Consider a nonsigular matrix $X \in \R^{n \times n}$ with bandwidth not greater than $B_X \geq 1$ induced by $(\G, \mathcal{I}, \mathcal{J})$. For constants $\bar{\sigma}_X \leq \bar{\sigma}(X)$ and $0 \leq \ubar{\sigma}_X \leq \ubar{\sigma}(X)$, the following holds
$$
\|X^{-1}_{[i][j]} \| \leq \frac{\bar{\sigma}_X}{\ubar{\sigma}^2_X}
\left(\frac{\bar{\sigma}_X^2 - \ubar{\sigma}^2_X}{\bar{\sigma}_X^2 + \ubar{\sigma}^2_X}\right)^{\left\lceil\frac{d_{\G}(i,j) - B_X}{2B_X}\right\rceil_+},
$$    
where $X^{-1}_{[i][j]} = X^{-1}_{\I_i, \J_j}$, $\bar{\sigma}(X), \ubar{\sigma}(X)$ denote the largest and smallest singular values of $X$, and $\left\lceil \cdot \right\rceil_+$ is the smallest non-negative integer that is greater than or equal to the argument.
\end{theorem}

This theorem states that the inverse of a graph-structured matrix has exponentially decaying components. The magnitude of the $i,j$-th component of its inverse decreases exponentially with respect to the distance of nodes $i,j$ in the graph $\mathcal{G}$. In addition, the rate of decrease depends on the conditioning of the matrix. 

\subsection{Decentralize scheme with overlap for graph-structured optimization problems}

Here we expose the \textit{synchronous coordination} scheme from~\cite{Shin2020-jc}. 

% explain what this scheme actually does, how it works, how the projections work
In a nutshell...

% main convergence result
\begin{theorem}
blablabla
\end{theorem}

\subsection{Decentralized computation of the coupling Jacobian}
Here we adapt the above scheme to our setting. 

\subsubsection{A bipartite graph}
In our case we have a bipartite graph, so we need to change a bit the way we think about projections

\subsubsection{Adapting the result from Shin}

It does not apply directly to us because...

The modifications we make are X-fold. 

this yields the following theorem
\begin{theorem}[Adapted from Theorem 2 in~\cite{Shin2020-jc}]\label{th:convergence_rate}
Consider~\eqref{eq:coupling_gradients} and the decentralized scheme in~\eqref{eq:sync_coord} for a given set of node-associated constraint sets $\{\V_k^\omega\}_{k\in \V_p}$ and $\omega \geq 0$. Assume that the conditions of Lemma~\ref{lemma:Lkw_invertible} are verified. Then the sequence generated by~\eqref{eq:coupling_gradients} satisfies
\begin{align}
    \|y^{(t)} - y^\star \|_{\infty} \leq \alpha^t \|y^{(0)} - y^\star \|_\infty,
\end{align}
where the convergence rate $\alpha$ is defined by
\begin{align}
    \label{eq:alpha}
   \alpha := \max_{k \in \V_p} \frac{R_k \bar{\sigma}_k}{\ubar{\sigma}^2_k}  
   \left(
   \frac{\bar{\sigma}^2_k - \ubar{\sigma}^2_k}{\bar{\sigma}_k^2 + \ubar{\sigma}_k^2}
   \right)^{\left\lceil(\omega+1)/B_{\lhs_k^\omega} - 1\right\rceil_+},
\end{align}
with $\bar{\sigma}^2_k$ and $\ubar{\sigma}^2_k$ the largest and smallest singular values of $\lhs_k^\omega$, respectively, and 
$R_k := \sum_{i \in \V_k^\omega, j \in \V \setminus \V_k^\omega} |(\lhs^\omega_{-k})_{i,j}|$.
\end{theorem}

The above result is a restatement of Theorem 2 in~\cite{Shin2020-jc}, without the assumption that the matrix be PD. As most steps in the proof remain unchanged, we do not rewrite it here entirely. We discuss the main differences in Appendix~\ref{proof:convergence_rate}.

The sequence~\eqref{eq:sync_coord} defines a scheme with linear convergence to solve~\eqref{eq:coupling_gradients}. The convergence rate $\alpha$ decreases exponentially with $\omega$. We note that for a given value of $\omega$, the conditioning as well as the graph-induced structure of the system will also impact $\alpha$. However, larger values of $\omega$ will come at a cost of more expensive communication, as more data needs to be exchanged both for constructing the projection matrices $\lhs_k^\omega, \lhs_{-k}^\omega, q_k^\omega$ and for the exchange of information at every iteration. In addition, the computational cost of one iteration of~\eqref{eq:sync_coord} increases with $\omega$. However, as $S_k^\omega$ remains unchanged with iterations, the factorization of $\lhs_k^\omega$ can be stored and does not need to be recomputed every time. 

==> body/5.Applications.tex <==
\section{Applications}\label{sec:applications}

The generality of the formulation of Problem~\ref{pbm:CCOP} makes it amenable to represent a host of practical problems. In this Section, we briefly discuss the advantages of the proposed framework for sensitivity analysis and illustrate them for distributed bi-level optimization.


\subsection{Sensitivity analysis of large-scale, weakly-coupled systems}

Quantifying the sensitivities of model solutions to parameters is a scientific discipline in itself that has many implications in systems analysis and modeling~\cite{Razavi2021-nf}. For instance, locational marginal emissions are effectively sensitivities of emissions to energy demand in a power system~\cite{Fuentes_Valenzuela2023-dj}. Resource allocation is a class of problems that consists in multiple participants sharing a limited number of resources and has very wide application domains~\cite{Patriksson2008-cu}. Effectively, resource allocation problems are \textit{constraint-coupled} problems and fit directly in the framework of Problem~\ref{pbm:CCOP}. Many solution methods exist that take advantage of this inherent structure~\cite{Falsone2017-zb, Falsone2020-pr, Su2022-kl, Shorinwa_undated-ay}. In addition, the potentially limited number of resources and large number of participants often makes those systems weakly coupled. As discussed in Section~\ref{sec:complexity}, sensitivity computation in large-scale weakly-coupled systems can be sped up dramatically with the proposed framework.

% To illustrate the computational benefits of our approach in the context of resource allocation problems, we apply decentralized implicit differentiation to the PEVs charging problem in~\cite{Vujanic2016-wj}. In this problem, $N$ PEVs are connected to the grid and require a minimum amount of charging overnight. The problem consists in determining when to charge each vehicle, subject to minimum and maximum total power requirements, so as to minimize system costs. Details, as well as numerical values used for the experiment are provided in~\cite{Vujanic2016-wj}. We consider the charging-only case, like in~\cite{Falsone2017-zb}.

% Sensitivity analysis can be relevant in this case to estimate the sensitivities of the charging schedule or power injections to, e.g., electricity costs, individual battery capacities, charging rates, etc. For instance, such metrics can be important in the optimal design of those systems~\cite{Degleris2021-vb} or in the quantification of marginal emissions rates~\cite{Fuentes_Valenzuela2023-dj}. This problem is particularly well suited to the framework of this paper. Indeed, the number of coupling constraints is $2T$, where $T$ is the number of timesteps in the optimization problem. It is fixed, regardless of the number of vehicles involved. In addition, subproblems are all defined by individual battery dynamics and contain a significant number of constraints, leading to a small value of the coupling ratio $\rho$. Simulation results are reported in Fig~\ref{fig:battery_model}. The weakly coupled structure of this problem leads to significant speed-ups as soon as a few hundred batteries are involved (see Panel A). Granular sensitivity metrics can therefore be extracted as a fraction of the computational cost. For instance, one can obtain the sensitivity of power injections at every battery with respect to the minimum and maximum total power requirements. Effectively, this informs on how a given battery charging schedule would vary as a function of those power bounds. In Panel B, 10 power injection trajectories for the 200-battery case and the cost signal in Fig.~\ref{supp_fig:cost} are represented. As expected, power injection is minimized when costs peak. This leads to interesting sensitivity landscape for the population of batteries. The sensitivity to the maximum (resp. minimum) total power injection bound is reported in Panel C (resp. D). First, there is a clear gradient in sensitivities throughout the simulation, implying that some batteries are significantly more sensitive than others to those power bounds even if they apply to the sum of individual injections. Second, there are two timepoints where sensitivities increase dramatically in magnitude, indicating a localized sharp response of the system to any change in those global coupling constraints. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{Figures/BatteryModel/BatteryModels.pdf}
%     \caption{Sensitivity computation for the battery model of~\cite{Falsone2017-zb}. (A) Speedup as a function of the number of vehicles involved in the problem. (B) 10 representative examples out of 200 battery power injection trajectories. (C, D) Quantiles of battery sensitivities with respect to maximum (C) and minimum (D) total power injection.
%     Parameter values used in this simulation are the same as in~\cite{Vujanic2016-wj}.
%     }
%     \label{fig:battery_model}
% \end{figure}


\subsection{Distributed bi-level optimization with arbitrary constraints}

A decentralized framework for gradient estimation opens the door to decentralized bi-level optimization. Indeed, let us consider a bilevel problem of the form

\begin{problem}[Separable bi-level problem]
\begin{align*}
   \min_{\theta} & \sum_i^N g_i(\theta_i, x_i^\star(\theta)) \\
    \text{s.t. }  \mathrm{x}^\star(\theta) = & \arg\min_{x_i} \sum_i^N f_i^0(x_i, \theta_i) \\ 
    & x_i \in \mathcal{C}_i(\theta_i)\\
    &\mathrm{x} \in \mathcal{D}(\theta_c)
\end{align*}
\end{problem}

Different methods exist for solving bi-level problems~\cite{Sinha2018-nh}, among which gradient-based methods are the most prevalent. In these settings, estimating the gradient of the outer-level problem can be expensive and difficult to distribute. Once this gradient has been estimated, every subproblem can update its local parameter with the following gradient-descent update
% \begin{align}
%     \theta_i^{k+1} &= \theta_i^k - \gamma^k \left(\partial_{\theta_i} g_i(\theta_i, x_i(\theta)) + \partial_{x_i}g_i(\theta_i, x_i(\theta))\partial_{\theta_i}x_i^\star(\theta)\right). 
% \end{align}
\begin{align}
    \theta_i^{k+1} &= \theta_i^k - \gamma^k \left(D_{\theta_i} g_i + D_{x_i}g_iD_{\theta_i}x_i^\star\right). 
\end{align}
The outer-level gradient, sometimes called \textit{hypergradient}, involves the Jacobian of the solution to the lower-level problem and can be readily estimated with our approach. Therefore, decentralized gradient computation opens the door to decentralized bi-level optimization for a broad class of problems. 

% comparison with previous work
% The other papers in distributed bi level optimization aim at inverting the full problem. This (i) only works for unconstrained problems, otherwise they should include constraint equations and (ii) is not what you're doing. What you're doing is approximating a correction term. I think it'd be nice to explain what previous works does, a bit like in ~\cite{Chen2022-pn}. And to explicitly say how your formulation is different in the case where the system is unconstrained. It is often written that the total hypergradient is not the average hypergradient... \textbf{but} it is not written that it is the local gradient + a correction term. it would be nice to make this distinction


For instance, in the context where data is not centralized but rather distributed between different agents in a network, sensitive information sharing might be undesirable. However, one might still want to be able to fine-tune a model by leveraging the entire dataset. In addition to computational efficiencies discussed in the previous section, a decentralized framework has the advantage of avoiding sharing sensitive information between subproblems. Hyperparameter optimization is one common application of this setting in machine learning~\cite{Franceschi2017-ub}. We illustrate our approach on decentralized hyperparameter optimization for Support Vector Machines (SVMs). SVMs consist in finding the maximum-margin separating hyperplane between two classes, and can be formulated as the following convex optimization problem
\begin{align*}
    \min_{w, b, \xi_{in}} & \lambda\| w\|_2^2 + \sum_{n=1}^{N} \sum_{i = 1}^{M_n} \xi_{ni} &\\ 
    \text{s.t. } & y_{ni}(w^Tx_{ni} + b) \geq 1-\xi_{in},&\ n=1...N, i=1...M_n\\
    & \xi_{ni} \geq 0,&\ n=1...N, i=1...M_n
\end{align*}
where the data is split is $N$ datasets, each with a total of $M_n$ datapoints. In the above formulation, the regularization parameter $\lambda$ is the main hyperparameter. If the $N$ datasets are distributed, a \textit{consensus}-based formulation of the distributed problem is~\cite{Forero2010-ek}
\begin{align*}
    \min_{w_n, b_n, \xi_{in}} & \sum_{n=1}^N \left(\frac{\lambda}{N} \|w_n\|_2^2 +  \sum_{i = 1}^{M_n} \xi_{ni}\right) &\\ 
    \text{s.t. } & y_{ni}(w^Tx_{ni} + b) \geq 1-\xi_{in},&\ n=1...N, i=1...M_n,\\
    & \xi_{ni} \geq 0,&\ n=1...N, i=1...M_n,\\
    & w_n = w_m, b_n = b_m & n \neq m.
\end{align*}
SVMs are often formulated and solved in dual form to enable the use of kernels of arbitrary complexity. However, it can be efficient to keep the primal form if, e.g., the number of features is small compared to the number of datapoints~\cite{Stolpe2016-tr}. 

Over the years, several efficient methods to solve SVMs in a distributed manner have been proposed~\cite{Forero2010-ek, Dutta2022-oe}, as well as gradient-based methods for hyperparameter optimization~\cite{Sathiya_Keerthi2006-su, Jiang2020-wr}. In this example, we extend those gradient-based methods to the decentralized setting. We consider the problem of leveraging data distributed between 10 agents in order to fit and tune an SVM model. For every value of the hyperparameter $\lambda$, the consensus-based formulation above is solved, ensuring that each agent has, at optimality, a copy of the optimal weights and bias vectors $w^\star, b^\star$. Then, the gradients $D_\lambda w^\star, D_\lambda b^\star$ are computed with our approach. Again, we assume the presence of a central node that gathers all local Jacobians and computes the coupling Jacobian. Local validation loss gradients can then be computed, before aggregating them and accordingly updating the hyperparameter $\lambda$ via gradient-descent with momentum. 

Results are presented in Fig.~\ref{fig:SVM}. First, we note that the hyperparameter $\lambda$ converges to one minimum corresponding to that obtained via grid search (Fig.~\ref{fig:SVM:val_loss_tot_landscape}). While this value $\lambda^\star$ minimizes the \textit{total} validation loss, it might of course not minimize individual validation losses. In Fig.~\ref{fig:SVM:val_loss_i}, one clearly sees this effect. This consensus, both in the optimization variables and in the hyperparameters, is achieved without any data exchange between the different agents.

\begin{figure}[ht]
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/SVM/val_loss_tot_landscape.png}
         \caption{Total validation loss as a function of the hyperparameter $\lambda$. Blue dotted line: validation loss obtained via grid search. Red line: optimization trajectory via gradient descent.
         Green crosses: starting and ending point of the optimization.
         }
         \label{fig:SVM:val_loss_tot_landscape}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/SVM/val_loss_i.png}
         \caption{Individual validation losses for each of the $N=10$ agents in the SVM example, as a function of the iteration number $k$.}
         \label{fig:SVM:val_loss_i}
     \end{subfigure}
    \caption{Distributed hyperparameter optimization for SVMs.}
    \label{fig:SVM}
\end{figure}


% \subsection{Comparison with the literature}
% It would be nice to discuss how the approach compares with other ways of doing distributed bilevel optimization
